RTNN: Accelerating Neighbor Search Using Hardware Ray Tracing

Neighbor search is of fundamental important to many engineering and science fields such as physics simulation and computer graphics. This paper proposes to formulate neighbor search as a ray tracing problem and leverage the dedicated ray tracing hardware in recent GPUs for acceleration. We show that a naive mapping under-exploits the ray tracing hardware. We propose two performance optimizations, query scheduling and query partitioning, to tame the inefficiencies. Experimental results show 2.2X -- 65.0X speedups over existing neighbor search libraries on GPUs. The code is available at https://github.com/horizon-research/rtnn.

==> future.tex <==
\section{Limitations and Future Work}
\label{sec:future}

While using BVH for neighbor search can in theory be generalized to any dimension, our current implementation is limited to 3D (or lower), fundamentally because the RT cores support only 3D BVHs (rightly so since rendering is the main target). Tree-based searches are known to be inefficient in higher dimensions anyways due to the curse of dimensionality~\cite{??}. Thus, our algorithm is unlikely to be used for high-dimensional neighbor searches even if future RT cores support high-dimensional BVHs.

Our algorithm is naturally amenable to approximate neighbor search (ANN). In particular, in the two main steps in our algorithm (\Sec{sec:idea:basic}) Step 2 is much more costly than Step 1, so if we can skip Step 2 by not performing ray-sphere test we can gain lots of performance. This is possible if we accept any neighbor that is within the AABB even though it is not within the sphere. This provides a hard error bound.

